It's Always 10:10: Reference Images Break a Bias That Prompts Only Dent

Text-to-image models appear to reproduce the habits of the photographs they learned from. Analog clocks are an extreme case: in advertising, watches almost always show 10:10, and generated clocks return to 10:10 even when another time is requested. We measure this bias and test three ways of overcoming it on 52 models available on the Magnific platform, with a replication on Higgsfield. Every image shows three identical clocks that must show 2:35, 6:50 and 11:20. The description of the object is fixed and only the request about the time changes: no time (A), the time in digits (B), the hand positions described by construction relative to the dial numerals (C), or the same description plus a drawn reference dial (D). Two AI readers read all 1,799 images blind from coded copies, with a third reader and the author settling disagreements (dial-level agreement 96.0% and 97.3%). With no time requested, 67% of the images have all three clocks at 10:10. On the 20 current models, all three clocks are correct in 34% of the images with digits, 30% with the hands described in words and 75% with the reference dial (D-B: +37 points, 95% CI +28 to +45); we found no evidence that describing the hands in words beats the digits (C-B: -4 points, CI -10 to +1). The replication on the 12 models shared by both platforms gives the same picture (B 54%, C 50%, D 81%). Writing the time reduces the bias but leaves two thirds of the images of the 20 current models with at least one wrong clock; adding a drawn reference raises full accuracy to three quarters and almost eliminates images entirely at 10:10. We release all images, prompts, raw readings and a script that recomputes every result.

==> tables/errors.tex <==
% generated by make_numbers.py
Correct & 0\% (0) & 43\% (231) & 46\% (250) & 83\% (403) \\
10:10 & 74\% (400) & 25\% (136) & 22\% (120) & 5\% (23) \\
Another clock's time & 0\% (0) & 1\% (4) & 1\% (4) & 0\% (1) \\
Hands swapped & 0\% (0) & 5\% (26) & 8\% (44) & 3\% (14) \\
Hands overlapping & 0\% (0) & 3\% (14) & 1\% (6) & 0\% (0) \\
Other error & 0\% (0) & 23\% (123) & 21\% (112) & 9\% (45) \\
Other time (A only) & 26\% (139) & 0\% (0) & 0\% (0) & 0\% (0) \\
Unreadable & 0\% (1) & 1\% (6) & 1\% (4) & 0\% (0) \\
\midrule
Dials ($N$) & 540 & 540 & 540 & 486 \\


==> tables/models.tex <==
% generated by make_numbers.py
GPT 2.5 Flare & 6/27 & 9/9 & 9/9 & 9/9 & 20/54 & 18/18 & 18/18 & 18/18 \\
GPT 2.5 Sunburst & 4/27 & 9/9 & 9/9 & 9/9 & 8/54 & 18/18 & 18/18 & 18/18 \\
Seedream 5 Pro & 24/27 & 9/9 & 6/9 & 9/9 & 46/54 & 18/18 & 16/18 & 18/18 \\
Grok Imagine 2.0 & 21/27 & 8/9 & 8/9 & 8/9 & 33/54 & 15/18 & 12/18 & 16/18 \\
Nano Banana 2.1 & 22/27 & 7/9 & 4/9 & 9/9 & 46/54 & 16/18 & 14/18 & 18/18 \\
Seedream 5 Flash & 21/27 & 6/9 & 7/9 & 9/9 & 48/54 & 16/18 & 14/18 & 18/18 \\
Qwen Image 3.0 Pro & 27/27 & 5/9 & 4/9 & 9/9 & \multicolumn{4}{c}{not on Higgsfield} \\
Nano Banana 2 & 25/27 & 6/9 & 4/9 & 6/9 & 42/54 & 9/18 & 7/18 & 13/18 \\
MAI Image 2.5 & 27/27 & 0/9 & 0/9 & 9/9 & \multicolumn{4}{c}{not on Higgsfield} \\
Seedream 5 Lite & 18/27 & 0/9 & 0/9 & 9/9 & \multicolumn{4}{c}{not on Higgsfield} \\
Luma Uni-1.1 & 25/27 & 0/9 & 1/9 & 8/9 & \multicolumn{4}{c}{not on Higgsfield} \\
Flux.3 Image & 27/27 & 0/9 & 0/9 & 7/9 & 53/54 & 0/18 & 0/18 & 8/18 \\
Ideogram 4.5 & 6/27 & 0/9 & 0/9 & 7/9 & 2/54 & 0/18 & 0/18 & 17/18 \\
Nano Banana 2 Lite & 24/27 & 2/9 & 1/9 & 5/9 & 43/54 & 3/18 & 2/18 & 7/17 \\
Flux.2 Pro & 27/27 & 0/9 & 0/9 & 4/9 & \multicolumn{4}{c}{not on Higgsfield} \\
Flux.2 Max & 27/27 & 0/9 & 0/9 & 3/9 & \multicolumn{4}{c}{not on Higgsfield} \\
Nano Banana Pro & 24/27 & 0/9 & 1/9 & 1/9 & 54/54 & 3/18 & 7/18 & 8/18 \\
Krea 2 & 21/27 & 0/9 & 0/9 & 0/9 & \multicolumn{4}{c}{not on Higgsfield} \\
Mystic 2.5 & 14/27 & 0/9 & 0/9 & -- & \multicolumn{4}{c}{not on Higgsfield} \\
Recraft V4.1 & 10/27 & 0/9 & 0/9 & -- & 37/54 & 0/18 & 0/18 & -- \\


==> tables/oldmodels.tex <==
% generated by make_numbers.py
Flux.1 Fast & 9/9 & 3/3 & Seedream 4 & 7/9 & 2/3 \\
Flux.1 Kontext Max & 9/9 & 3/3 & Cinematic & 6/9 & 2/3 \\
Flux.2 Flex & 9/9 & 3/3 & Flux.1 Realism & 6/9 & 2/3 \\
Flux.2 Klein & 9/9 & 3/3 & Ideogram 4 & 6/9 & 2/3 \\
GPT & 9/9 & 3/3 & Mystic 1.0 & 6/9 & 2/3 \\
GPT 1 HQ & 9/9 & 3/3 & Mystic 2.5 Fluid & 6/9 & 2/3 \\
Grok & 9/9 & 3/3 & Recraft V4 Pro & 6/9 & 2/3 \\
Ideogram & 9/9 & 3/3 & GPT 2 & 4/9 & 1/3 \\
Mystic 2.5 Flexible & 9/9 & 3/3 & Seedream 4 4K & 4/9 & 1/3 \\
Qwen & 9/9 & 3/3 & Flux.1 & 3/9 & 1/3 \\
Qwen Image 3.0 & 9/9 & 3/3 & Recraft V4 & 3/9 & 1/3 \\
Z-Image & 9/9 & 3/3 & Seedream 4.5 & 3/9 & 1/3 \\
Classic Fast & 8/9 & 0/3 & Classic & 1/9 & 0/3 \\
Flux.1 Kontext Pro & 8/9 & 2/3 & GPT 1.5 & 0/9 & 0/3 \\
Flux.1.1 & 7/9 & 2/3 & GPT 1.5 High & 0/9 & 0/3 \\
Nano Banana (prima versione) & 7/9 & 1/3 & P-Image Ideogram & 0/9 & 0/3 \\

